Privately Answering Counting Queries with Generalized Gaussian Mechanisms

We consider the problem of answering $k$ counting (i.e. sensitivity-1) queries about a database with $(\epsilon, \delta)$-differential privacy. We give a mechanism such that if the true answers to the queries are the vector $d$, the mechanism outputs answers $\tilde{d}$ with the $\ell_\infty$-error guarantee: $$\mathcal{E}\left[||\tilde{d} - d||_\infty\right] = O\left(\frac{\sqrt{k \log \log \log k \log(1/\delta)}}{\epsilon}\right).$$ This reduces the multiplicative gap between the best known upper and lower bounds on $\ell_\infty$-error from $O(\sqrt{\log \log k})$ to $O(\sqrt{\log \log \log k})$. Our main technical contribution is an analysis of the family of mechanisms of the following form for answering counting queries: Sample $x$ from a \textit{Generalized Gaussian}, i.e. with probability proportional to $\exp(-(||x||_p/\sigma)^p)$, and output $\tilde{d} = d + x$. This family of mechanisms offers a tradeoff between $\ell_1$ and $\ell_\infty$-error guarantees and may be of independent interest. For $p = O(\log \log k)$, this mechanism already matches the previous best known $\ell_\infty$-error bound. We arrive at our main result by composing this mechanism for $p = O(\log \log \log k)$ with the sparse vector mechanism, generalizing a technique of Steinke and Ullman.

==> lpq-deferred.tex <==
\section{Generalizations of $\mpq_\sigma$}\label{section:lpq}

In this section, we consider sampling $x$ with probability proportional to $\exp(-(\norm{x}_p / \sigma)^q)$ for $q \leq p$ instead of $\exp(-(\norm{x}_p / \sigma)^p)$. Most proofs in Section~\ref{section:lpp} and~\ref{section:sv} generalize readily to analyzing this mechanism. For brevity's sake, we only describe how to modify the proofs whose generalization is less clear. First, we show how to generalize Lemma~\ref{lemma:sigmachoice}:

\begin{lemma}\label{lemma:sigmachoice-generalized}
Let $\mpqq_\sigma$ be the mechanism such that $\mpqq_\sigma(d)$ samples $x \in \mathbb{R}^k$ with probability proportional to $\exp(-(\norm{x}_p / \sigma)^q)$ and outputs $\tilde{d} = d+x$. For $4 \leq p \leq \log k$ that is an even integer, $q \leq p, \epsilon \leq O(1), \delta \in [1/k^{\omega(1)}, 2^{-O(k / p)}]$, and

$$\sigma  = \Theta\left( \frac{k^{1/2 + 1/p - 1/q} \sqrt{p \log (1/\delta)}}{\epsilon} \right),$$

$\mpqq_\sigma$ is $(\epsilon, \delta)$-differentially private.
\end{lemma}
\begin{proof}

Recall we want to show:

$$\frac{\Pr[\mpqq_\sigma(d) = \tilde{d}]}{\Pr[\mpqq_\sigma(d+\Delta) = \tilde{d}]} = \frac{\exp(-(\norm{x}_p / \sigma)^q)}{\exp(-(\norm{x-\Delta}_p / \sigma)^q)} = \exp\left(\frac{\norm{x-\Delta}_p^q - \norm{x}_p^q}{\sigma^q}\right).$$

If $\norm{x - \Delta} \leq \norm{x}$, then trivially this is less than $e^\epsilon$, so we only need to bound this ratio for $x$ such that $\norm{x - \Delta} > \norm{x}$. Analyzing the difference in norms, we have:

$$\norm{x-\Delta}_p^q - \norm{x}_p^q = (\norm{x-\Delta}_p^p)^{q/p} - (\norm{x}_p^p)^{q/p} = \int_{\norm{x}_p^p}^{\norm{x-\Delta}_p^p} \frac{q}{p} y^{q/p-1} \D{y} \leq $$
$$\int_{\norm{x}_p^p}^{\norm{x - \Delta}_p^p} \frac{q}{p} (\norm{x}_p^p)^{q/p-1} \D{y} = \frac{q}{p} \cdot \norm{x}_p^{q-p} \cdot (\norm{x-\Delta}_p^p - \norm{ x }_p^p).$$

In the inequality, we are using that $q \leq p$ and so the integrand is maximized when $y = \norm{x}_p^p$. By Lemma~\ref{lemma:lppdifference} we now have with probability $1 - \delta/2$ for a sufficiently large constant $c_1$:

$$\norm{x - \Delta}_p^q - \norm{x}_p^q \leq cq k^{1/p - 1/2}\sqrt{p \log (1/\delta)}\norm{x}_p^{q-1} + cqk^{\frac{p}{2}}p \norm{x}_p^{q-p}.$$

$\norm{x}_p^q$ has distribution $Gamma(k/q)$ and so by a Gamma tail bound with probability at least $1 - e^{-.001k/q} > 1 - \delta/2$, $\norm{x}_p$ is contained in $[\sigma \left(\frac{k}{2q}\right)^{1/q}, \sigma \left(\frac{2k}{q}\right)^{1/q}]$. Then by a union bound, with probability $1 - \delta$:

$$\frac{\norm{x - \Delta}_p^q - \norm{x}_p^q}{\sigma^q} \leq \frac{2cq^{1/q} k^{1/2 +1/p - 1/q}\sqrt{p \log (1/\delta)}}{\sigma} + \frac{2^{p/q-1}cq^{p/q}k^{\frac{p}{2}+1-\frac{p}{q}}p}{\sigma^p}.$$

Noting that $n^{1/n}$ is contained within $[1, e^{1/e}]$ for all $n \geq 1$, letting 

$$\sigma = \Theta\left( \max\left\{\frac{k^{1/2 + 1/p - 1/q} \sqrt{p \log (1/\delta)}}{\epsilon}, \frac{k^{1/2 + 1/p - 1/q} }{\epsilon^{1/p}}\right\} \right) $$
$$ = \Theta\left( \frac{k^{1/2 + 1/p - 1/q} \sqrt{p} \sqrt{\log (1/\delta)}}{\epsilon} \right),$$

we get that $\frac{\norm{x - \Delta}_p^q - \norm{x}_p^q }{\sigma^q} \leq \epsilon$ as desired.
\end{proof}

The proof of a generalization of Theorem~\ref{thm:main-1} follows almost exactly the same as the original proof, since $\norm{x}_p^q$ is now distributed as $Gamma(k/q)$, and achieves the same error bound as a function of $p$.

We can also prove a generalization of Theorem~\ref{thm:main-2} (with the same error bound as a function of $p$) that holds for a family of mechanisms which each start by sampling $x$ with probability proportional to $\exp(-(\norm{x}_p/\sigma)^q)$ before applying sparse vector. The coordinates of $x$ sampled this way are not independent if $p \neq q$, but we can the indicators for whether they exceed $\alpha_{SV}/2$ as defined in the proof of Theorem~\ref{thm:main-2} are negatively associated, which lets us use a generalized Chernoff bound in the proof of Theorem~\ref{thm:main-2}:
\begin{definition}
A set of random variables $X_1, X_2, \ldots X_k$ are negatively associated if for any disjoint subsets $S, T$ of the random variables and any functions $f, g$ of $S, T$ respectively that are both monotonically increasing:

$$\ex[f(S) g(T)] \leq \ex[f(S)] \ex[g(T)].$$
\end{definition}

Traditionally the definition of negative association requires also considering the case where both $f, g$ are monotonically decreasing. However, the above inequality is equivalent for $f, g$ and  $-f, -g$ (which are monotonically increasing if $f, g$ are monotonically decreasing), so this is not necessary.

\begin{lemma}[Chernoff Bound for Negatively Associated Bernoullis \cite{DubhashiR96}]\label{lemma:chernoffna-generalized}
Let $X_1, X_2, \ldots X_k$ be negatively associated random variables with support $\{0, 1\}$. Let $\mu = \ex\left[\sum_{i \in [k]} X_i\right]$. Then for $t \in [0, 1]$, we have:
$$\Pr\left[\left|\sum_{i \in [k]} X_i - \mu\right| \geq t \mu\right] \leq 2 \cdot \exp\left(-\frac{t^2 \mu}{3}\right).$$
\end{lemma}

\begin{lemma}\label{lemma:spherecapnegative}
Let $x$ be chosen uniformly at random from the $k$-dimensional $\ell_p$-sphere with arbitrary radius, i.e. the set of points with $\norm{x}_p = R$ for some $R$, for $p \geq 1$. Then the indicator random variables $\mathbb{I}[|x_i| \geq r \norm{x}_p]$ are negatively associated.
\end{lemma}
\begin{proof}
We will show that the random variables $|x_i|$ are negatively associated. The lemma follows since monotonically increasing functions of negatively associated random variables are negatively associated \cite{DubhashiR96}. For any subset $S$ of the $|x_i|$, conditional on the value $R_S = (\sum_{x_i \in S}|x_i|^p/\norm{x}_p^p)^{1/p}$, we have that the $|x_i|$ in $S$ (resp. the $|x_i$ not in $S$) are distributed as the $|x_i|$ given from a uniform sample from the $|S|$-dimensional (resp. $(k-|S|)$-dimensional) $\ell_p$-sphere of radius $R_S$ (resp. $(1-R_S^p)^{1/p}$. These distributions are of course identical up to rescaling by the radius of the sphere. 

It follows that for any monotonically increasing function $f$ of $S$, $\ex_S[f(S) | R_S]$ is a monotonically increasing function of $R_S$, since for any $0 \leq r_1 \leq r_2 \leq 1$ there is a coupling between $S_1$ defined as the distribution of $S$ conditional on $R_S = r_1$ and $S_2$ defined as the distribution of $S$ conditional on $R_S = r_2$ such that under this coupling, $S_1$'s $|x_i|$ values are all less than $S_2$'s corresponding $|x_i|$ values and thus $\Pr[f(S_1) \leq f(S_2)] = 1$ (namely, the coupling is just that $S_2$ is $S_1$ rescaled by $r_2/r_1$). Using a similar argument, for any subset $T$ of the $x_i$ that is disjoint from $S$ and any monotonically increasing function $g$ of $T$, we can conclude that $\ex_T[g(T) | R_S]$ is monotonically decreasing in $R_S$, and thus that $\ex[f(S) | R_S]$ is negatively correlated with $\ex[g(T) | R_S]$. Finally, conditional on $R_S$, $f(S)$ and $g(T)$ are identically distributed. Then we have:
$$\ex_{R_S}[\ex_S[f(S) | R_S] \ex_T[g(T) | R_S]] \leq \ex[\ex_S[f(S)|R_S]] \ex_T[\ex[g(T)|R_S]] \implies $$
$$\ex_{R_S}[\ex_{S, T}[f(S) g(T) | R_S]] \leq \ex_{R_S}[\ex_S[f(S)|R_S]] \ex_{R_S}[\ex_T[g(T)|R_S]] \implies $$
$$\ex_{\{x_i\}}[f(S) g(T)] \leq \ex_{\{x_i\}}[f(S)] \ex_{\{x_i\}}[g(T)].$$

Here we start by using negative correlation, then independent of $f(S), g(T)$ conditioned on $R_S$, then the law of total expectation. This shows the random variables $|x_i|$ are negatively associated. 
\end{proof}

To generalize the proof of Theorem~\ref{thm:main-2} to the setting where the $x_i$ are not independent, we first condition on the norm of $x$, ignoring the low-probability event where it is large, and then use Lemma~\ref{lemma:spherecapnegative} to replace the Chernoff bound in the proof.
